Near-optimal hierarchical matrix approximation from matrix-vector products

We describe a randomized algorithm for producing a near-optimal hierarchical off-diagonal low-rank (HODLR) approximation to an $n\times n$ matrix $\mathbf{A}$, accessible only though matrix-vector products with $\mathbf{A}$ and $\mathbf{A}^{\mathsf{T}}$. We prove that, for the rank-$k$ HODLR approximation problem, our method achieves a $(1+\beta)^{\log(n)}$-optimal approximation in expected Frobenius norm using $O(k\log(n)/\beta^3)$ matrix-vector products. In particular, the algorithm obtains a $(1+\varepsilon)$-optimal approximation with $O(k\log^4(n)/\varepsilon^3)$ matrix-vector products, and for any constant $c$, an $n^c$-optimal approximation with $O(k \log(n))$ matrix-vector products. Apart from matrix-vector products, the additional computational cost of our method is just $O(n \operatorname{poly}(\log(n), k, \beta))$. We complement the upper bound with a lower bound, which shows that any matrix-vector query algorithm requires at least $\Omega(k\log(n) + k/\varepsilon)$ queries to obtain a $(1+\varepsilon)$-optimal approximation. Our algorithm can be viewed as a robust version of widely used "peeling" methods for recovering HODLR matrices and is, to the best of our knowledge, the first matrix-vector query algorithm to enjoy theoretical worst-case guarantees for approximation by any hierarchical matrix class. To control the propagation of error between levels of hierarchical approximation, we introduce a new perturbation bound for low-rank approximation, which shows that the widely used Generalized Nystr\"om method enjoys inherent stability when implemented with noisy matrix-vector products. We also introduce a novel randomly perforated matrix sketching method to further control the error in the peeling algorithm.

==> imgs/hard_example.tex <==
\begin{NiceMatrixBlock}[]\footnotesize
$\vec{A}^{(3)} =$ \scalebox{.7}{$
\begin{NiceArray}{cccccccc}[hvlines,columns-width=6mm,cell-space-limits=8pt,rules/width=0.2pt]
    \Block[fill=black!25]{1-1}{}  & \Block[]{1-1}{\phantom{\vec{A}^{(3)}_{1,2}}} &\Block[]{2-2}{}  && \Block[]{4-4}{}  &&&\\
    \Block[fill=black!10]{1-1}{\vec{A}^{(3)}_{2,1}} & \Block[fill=black!25]{1-1}{} &&&&&&\\
    \Block[]{2-2}{} && \Block[fill=black!25]{1-1}{}& \Block[]{1-1}{\phantom{\vec{A}^{(3)}_{3,4}}} &&&& \\
     && \Block[fill=black!10]{1-1}{\vec{A}^{(3)}_{4,3}} & \Block[fill=black!25]{1-1}{}  &&&& \\
    \Block[]{4-4}{}  &\Block[]{1-1}{}&&& \Block[fill=black!25]{1-1}{}  & \Block[]{1-1}{\phantom{\vec{A}^{(3)}_{5,6}}} &\Block[]{2-2}{}  &  \\
     &&&& \Block[fill=black!10]{1-1}{\vec{A}^{(3)}_{6,5}} & \Block[fill=black!25]{1-1}{}  && \\
     &&&& \Block[]{2-2}{}  && \Block[fill=black!25]{1-1}{}  & \Block[]{1-1}{\phantom{\vec{A}^{(3)}_{7,8}}} \\
     &&&&&&\Block[fill=black!10]{1-1}{\vec{A}^{(3)}_{8,7}}& \Block[fill=black!25]{1-1}{}     \end{NiceArray}
$}
\end{NiceMatrixBlock}

==> imgs/nbody.tex <==
\begin{tikzpicture}

    \fill[black!10] (0,-.2)  rectangle (2,.2);
    \fill[black!20] (2,-.2)  rectangle (4,.2);
    \fill[black!10] (4,-.2)  rectangle (6,.2);
    \fill[black!20] (8,-.2)  rectangle (10,.2);
    
    \draw[-] (-.3,0) -- (6.1,0);
    \draw[dotted] (6.1,0) -- (7.9,0);
    \draw[-] (7.9,0) -- (10.3,0);

    \foreach \x in {.1,.3,.6,.7,1.3,1.4,1.9,2.3,2.6,3.1,3.7,3.8,,4.2,4.4,4.8,5.1,5.2,5.8,8.3,8.4,8.9,9.4,9.8} {
        \filldraw[] (\x,0) circle (1.5pt);
    }

    \draw[<-] (.3,-.1) -- (.3,-.4) node[below]{$x_i$};
    \draw[<-] (9.4,-.1) -- (9.4,-.4) node[below]{$x_j$};

    \draw [decorate,decoration={brace,amplitude=5pt,raise=.25cm}]
  (0,0) -- (2,0) node[midway,yshift=.6cm]{$G_1$};
    \draw [decorate,decoration={brace,amplitude=5pt,raise=.25cm}]
  (2,0) -- (4,0) node[midway,yshift=.6cm]{$G_2$};
      \draw [decorate,decoration={brace,amplitude=5pt,raise=.25cm}]
  (4,0) -- (6,0) node[midway,yshift=.6cm]{$G_3$};
      \draw [decorate,decoration={brace,amplitude=5pt,raise=.25cm}]
  (8,0) -- (10,0) node[midway,yshift=.6cm]{$G_m$};
    
\end{tikzpicture}

\begin{NiceMatrixBlock}[]\footnotesize
\scalebox{.7}{$
\begin{NiceArray}{ccccc}[hvlines,columns-width=6mm,cell-space-limits=8pt,rules/width=0.2pt]
    \Block[fill=black!25]{1-1}{A_{1,1}} &&&& \Block[fill=black!25]{1-1}{A_{1,m}} \\ 
    & \Block[fill=black!25]{1-1}{A_{2,2}} &&& \\ 
    & \Block[fill=black!25]{1-1}{A_{2,2}} &&& \\ 
    & \Block[fill=black!25]{1-1}{A_{2,2}} &&& \\ 
    & \Block[fill=black!25]{1-1}{A_{2,2}} &&& \\ 
\end{NiceArray}
$}
\end{NiceMatrixBlock}


==> imgs/peeling_fig3.tex <==
\begin{tikzpicture}
    \node[] at (-.85,4.1) {\large$\vec{A}^{(3)} = $};
    
    \draw[] (0,0) rectangle (8,8);
    
    \draw[] (0,0) rectangle (4,4);
    \draw[] (4,4) rectangle (8,8);

    \draw[] (0,4) rectangle (2,6);
    \draw[] (2,6) rectangle (4,8);
    \draw[] (4,0) rectangle (6,2);
    \draw[] (6,2) rectangle (8,4);


    \foreach \x in {0,...,7}{
    \draw[dotted,line width=.25pt] (\x,0) -- (\x,8);
    \draw[dotted,line width=.25pt] (0,\x) -- (8,\x);
    }
    
    \draw[fill=black!10] (0,6) rectangle (1,7) node[pos=.5] {$\vec{A}^{(3)}_{2,1}$};
    \draw[fill=black!10] (1,7) rectangle (2,8) node[pos=.5,text=black!50] {$\vec{A}^{(3)}_{1,2}$};
    \draw[fill=black!10] (2,4) rectangle (3,5) node[pos=.5] {$\vec{A}^{(3)}_{4,3}$};
    \draw[fill=black!10] (3,5) rectangle (4,6) node[pos=.5,text=black!50] {$\vec{A}^{(3)}_{3,4}$};
    \draw[fill=black!10] (4,2) rectangle (5,3) node[pos=.5] {$\vec{A}^{(3)}_{6,5}$};
    \draw[fill=black!10] (5,3) rectangle (6,4) node[pos=.5,text=black!50] {$\vec{A}^{(3)}_{5,6}$};
    \draw[fill=black!10] (6,0) rectangle (7,1) node[pos=.5] {$\vec{A}^{(3)}_{8,7}$};
    \draw[fill=black!10] (7,1) rectangle (8,2) node[pos=.5,text=black!50] {$\vec{A}^{(3)}_{7,8}$};


    \draw[fill=black!20] (0,7) rectangle (1,8);
    \draw[fill=black!20] (1,6) rectangle (2,7);
    \draw[fill=black!20] (2,5) rectangle (3,6);
    \draw[fill=black!20] (3,4) rectangle (4,5);
    \draw[fill=black!20] (4,3) rectangle (5,4);
    \draw[fill=black!20] (5,2) rectangle (6,3);
    \draw[fill=black!20] (6,1) rectangle (7,2);
    \draw[fill=black!20] (7,0) rectangle (8,1);
\end{tikzpicture}
\hspace{1em}
\begin{tikzpicture}
    \node[] at (-.85,4.1) {\large$\vec{\Omega}^{+} = $};

    \draw[] (0,0) rectangle (1,8);
    
    \foreach \x in {1,3,5,7}{
    \draw[fill=black!10] (0,{8-\x}) rectangle (1,{8-\x+1}) node[pos=.5] {$\vec{\Omega}_{\x}$};
    }
\end{tikzpicture}
\hspace{1em}
\begin{tikzpicture}
    \node[] at (-.85,4.1) {\large$\vec{\Psi}^{-} = $};

    \draw[] (0,0) rectangle (1,8);
    
    \foreach \x in {2,4,6,8}{
    \draw[fill=black!10] (0,{8-\x}) rectangle (1,{8-\x+1}) node[pos=.5] {$\vec{\Psi}_{\x}$};
    }
\end{tikzpicture}

==> imgs/peeling_fig_nicearray.tex <==
\begin{NiceMatrixBlock}[]\footnotesize
$\vec{A}^{(3)} =$ \scalebox{.7}{$
\begin{NiceArray}{cccccccc}[hvlines,columns-width=6mm,cell-space-limits=8pt,rules/width=0.2pt]
    \Block[fill=black!25]{1-1}{}  & \Block[fill=black!10]{1-1}{\vec{A}^{(3)}_{1,2}} &\Block[]{2-2}{}  && \Block[]{4-4}{}  &&&\\
    \Block[fill=black!10]{1-1}{\vec{A}^{(3)}_{2,1}} & \Block[fill=black!25]{1-1}{} &&&&&&\\
    \Block[]{2-2}{} && \Block[fill=black!25]{1-1}{}& \Block[fill=black!10]{1-1}{\vec{A}^{(3)}_{3,4}} &&&& \\
     && \Block[fill=black!10]{1-1}{\vec{A}^{(3)}_{4,3}} & \Block[fill=black!25]{1-1}{}  &&&& \\
    \Block[]{4-4}{}  &\Block[]{1-1}{}&&& \Block[fill=black!25]{1-1}{}  & \Block[fill=black!10]{1-1}{\vec{A}^{(3)}_{5,6}} &\Block[]{2-2}{}  &  \\
     &&&& \Block[fill=black!10]{1-1}{\vec{A}^{(3)}_{6,5}} & \Block[fill=black!25]{1-1}{}  && \\
     &&&& \Block[]{2-2}{}  && \Block[fill=black!25]{1-1}{}  & \Block[fill=black!10]{1-1}{\vec{A}^{(3)}_{7,8}} \\
     &&&&&&\Block[fill=black!10]{1-1}{\vec{A}^{(3)}_{8,7}}& \Block[fill=black!25]{1-1}{}     \end{NiceArray}
$}
    \hspace{1em}
    $\vec{\Omega}^+ = $ \scalebox{.7}{$
    \begin{NiceArray}{c}[hvlines,columns-width=6mm,cell-space-limits=8pt,rules/width=0.2pt]
    \Block[fill=black!10]{1-1}{\vec{\Omega}^+_{1}}\\
    \phantom{\vec{\Omega}^+_{3,2}}\\
    \Block[fill=black!10]{1-1}{\vec{\Omega}^+_{3}}\\
    \phantom{\vec{\Omega}^+_{3,2}}\\
    \Block[fill=black!10]{1-1}{\vec{\Omega}^+_{5}}\\
    \phantom{\vec{\Omega}^+_{3,2}}\\
    \Block[fill=black!10]{1-1}{\vec{\Omega}^+_{7}}\\
    \phantom{\vec{\Omega}^+_{3,2}}\\
    \end{NiceArray}
    $}
    \hspace{.5em}
    $\vec{\Psi}^- = $ \scalebox{.7}{$
    \begin{NiceArray}{c}[hvlines,columns-width=6mm,cell-space-limits=8pt,rules/width=0.2pt]
    \phantom{\vec{\Psi}^+_{3,2}}\\
    \Block[fill=black!10]{1-1}{\vec{\Psi}^-_{2}}\\
    \phantom{\vec{\Psi}^+_{3,2}}\\
    \Block[fill=black!10]{1-1}{\vec{\Psi}^-_{4}}\\
    \phantom{\vec{\Psi}^+_{3,2}}\\
    \Block[fill=black!10]{1-1}{\vec{\Psi}^-_{6}}\\
    \phantom{\vec{\Psi}^+_{3,2}}\\
    \Block[fill=black!10]{1-1}{\vec{\Psi}^-_{8}}\\
    \end{NiceArray}
    $}
\end{NiceMatrixBlock}

==> imgs/step_l_fig.tex <==
\begin{NiceMatrixBlock}[]\footnotesize
$\vec{A} =$ \scalebox{.7}{$
\begin{NiceArray}{cccccccc}[hvlines,columns-width=6mm,cell-space-limits=8pt,rules/width=0.2pt,last-col,last-row]
    \Block[fill=black!25]{1-1}{}  & \Block[fill=black!10]{1-1}{\vec{A}_{1,2}} &\Block[tikz={pattern=dots, pattern color=black!50}]{2-2}{}  && \Block[tikz={pattern=dots, pattern color=black!50}]{4-4}{}  &&&\\
    \Block[fill=black!10]{1-1}{\vec{A}_{2,1}} & \Block[fill=black!25]{1-1}{} &&&&&&\\
    \Block[tikz={pattern=dots, pattern color=black!50}]{2-2}{} && \Block[fill=black!25]{1-1}{}& \Block[fill=black!10]{1-1}{\vec{A}_{3,4}} &&&& \\
     && \Block[fill=black!10]{1-1}{\vec{A}_{3,4}} & \Block[fill=black!25]{1-1}{}  &&&& \\
    \Block[tikz={pattern=dots, pattern color=black!50}]{4-4}{}  &\Block[tikz={pattern=crosshatch, pattern color = red!60}]{1-1}{}&&& \Block[fill=black!25]{1-1}{}  & \Block[fill=black!10,tikz={pattern=crosshatch, pattern color = green!60}]{1-1}{\vec{A}_{5,6}} &\Block[tikz={pattern=dots, pattern color=black!50}]{2-2}{}  &&j\pm1  \\
     &&&& \Block[fill=black!10]{1-1}{\vec{A}_{6,5}} & \Block[fill=black!25]{1-1}{}  && \\
     &&&& \Block[tikz={pattern=dots, pattern color=black!50}]{2-2}{}  && \Block[fill=black!25]{1-1}{}  & \Block[fill=black!10]{1-1}{\vec{A}_{7,8}} \\
     &&&&&&\Block[fill=black!10]{1-1}{\vec{A}_{8,7}}& \Block[fill=black!25]{1-1}{} \\
     &&&&&j \\
    \end{NiceArray}
$}
    \hspace{2em}
    $\vec{S}^- = $ \scalebox{.7}{$
    \begin{NiceArray}{ccc}[hvlines,columns-width=6mm,cell-space-limits=8pt,rules/width=0.2pt,last-col,last-row]
    \phantom{\vec{G}^+_{3,2}}&&\\
    &&\Block[fill=black!25,tikz={pattern=crosshatch, pattern color = red!60}]{1-1}{\vec{G}^+_{2,3}}&\\
    \phantom{\vec{G}^+_{3,2}}&&\\
    \Block[fill=black!25]{1-1}{\vec{G}^-_{1,4}}&&\\
    \phantom{\vec{G}^+_{3,2}}&&\\
    &&\Block[fill=black!25,tikz={pattern=crosshatch, pattern color = green!60}]{1-1}{\vec{G}^-_{6,3}}&j\\
    \phantom{\vec{G}^-_{3,2}}&&\\
    &\Block[fill=black!25]{1-1}{\vec{G}^-_{8,2}}\\
    &&\sigma
    \end{NiceArray}
    $}
\end{NiceMatrixBlock}
